Rethinking Sampling in 3D Point Cloud Generative Adversarial Networks

In this paper, we examine the long-neglected yet important effects of point sampling patterns in point cloud GANs. Through extensive experiments, we show that sampling-insensitive discriminators (e.g.PointNet-Max) produce shape point clouds with point clustering artifacts while sampling-oversensitive discriminators (e.g.PointNet++, DGCNN) fail to guide valid shape generation. We propose the concept of sampling spectrum to depict the different sampling sensitivities of discriminators. We further study how different evaluation metrics weigh the sampling pattern against the geometry and propose several perceptual metrics forming a sampling spectrum of metrics. Guided by the proposed sampling spectrum, we discover a middle-point sampling-aware baseline discriminator, PointNet-Mix, which improves all existing point cloud generators by a large margin on sampling-related metrics. We point out that, though recent research has been focused on the generator design, the main bottleneck of point cloud GAN actually lies in the discriminator design. Our work provides both suggestions and tools for building future discriminators. We will release the code to facilitate future research.

==> tex/07_impact.tex <==
%Authors are required to include a statement of the broader impact of their work, including its ethical aspects and future societal consequences. 
%Authors should discuss both positive and negative outcomes, if any. For instance, authors should discuss a) 
%who may benefit from this research, b) who may be put at disadvantage from this research, c) what are the consequences of failure of the system, and d) whether the task/method leverages
%biases in the data. If authors believe this is not applicable to them, authors can simply state this.
%Use unnumbered first level headings for this section, which should go at the end of the paper. {\bf Note that this section does not count towards the eight pages of content that are allowed.}

a) This work aims to build a better generative model for 3D point clouds. People caring about 3D shape synthesis and reconstruction may benefit from this research. A better generative model also provide priors for other perception tasks, e.g. localization, classification. Therefore, people who leverage 3D vision in their research or products may benefit from us as well, e.g. robotics, autonomous driving. 

b) This work focuses on the scientific problems of point cloud synthesis and doesn't directly deliver any product. However, as the fields that may benefit from our work, robotics and autonomous driving can potentially affect someone's job. We believe there is a low risk that our work may put someone at the disadvantages.

c) As our work can be used in various cases, it is hard to say the consequences of failure of our method. In most of the cases, it just generates inauthentic fake shapes. 

d) As a pure geometry generation task, our method considers the shape prior but not other social biases.
